AgentFL: Scaling LLM-based Fault Localization to Project-Level Context

Fault Localization (FL) is an essential step during the debugging process. With the strong capabilities of code comprehension, the recent Large Language Models (LLMs) have demonstrated promising performance in diagnosing bugs in the code. Nevertheless, due to LLMs' limited performance in handling long contexts, existing LLM-based fault localization remains on localizing bugs within a small code scope (i.e., a method or a class), which struggles to diagnose bugs for a large code scope (i.e., an entire software system). To address the limitation, this paper presents AgentFL, a multi-agent system based on ChatGPT for automated fault localization. By simulating the behavior of a human developer, AgentFL models the FL task as a three-step process, which involves comprehension, navigation, and confirmation. Within each step, AgentFL hires agents with diversified expertise, each of which utilizes different tools to handle specific tasks. Particularly, we adopt a series of auxiliary strategies such as Test Behavior Tracking, Document-Guided Search, and Multi-Round Dialogue to overcome the challenges in each step. The evaluation on the widely used Defects4J-V1.2.0 benchmark shows that AgentFL can localize 157 out of 395 bugs within Top-1, which outperforms the other LLM-based approaches and exhibits complementarity to the state-of-the-art learning-based techniques. Additionally, we confirm the indispensability of the components in AgentFL with the ablation study and demonstrate the usability of AgentFL through a user study. Finally, the cost analysis shows that AgentFL spends an average of only 0.074 dollars and 97 seconds for a single bug.

==> 3.motivation.tex <==
\section{Motivation}
\label{sec:motiv}

We motivate our approach through a real-world bug Lang-34 in the Defects4J-V1.2.0 \cite{just2014defects4j} benchmark, where the wide semantic gap between test failure information and problematic functionality impedes existing LLM-based technologies from reaching the expected fault location. As demonstrated in Figure \ref{fig:motiv}, the test \texttt{testObjectCycle} failed due to the usage of thread local in \texttt{ToStringStyle.java} which triggers a memory leak in the container environment\footnote{https://issues.apache.org/jira/browse/LANG-586}. The bug is fixed by modifying two methods \texttt{isRegistered} (omitted in Figure \ref{fig:motiv}) and \texttt{getRegistry}.

{\bf Demand for Execution Information.}
A basic inference from the example is that it is impossible to locate the buggy method given merely the test failure information, because the text of the buggy method \texttt{getRegistry} does not even appear in the test code or the error stack trace.
It can be seen from line 7 in the error stack trace that the unmet assert statement \texttt{assertNull} lies in \texttt{TestCase.java} rather than the test class \texttt{ToStringBuilderTest}.
Moreover, The failed test \texttt{ToStringBuilderTest::testObjectCycle} aims at testing the functional correctness of class \texttt{ToStringBuilder}, however, the fixed methods hide in another class \texttt{ToStringStyle} on the execution path.
In reality, previous studies have discovered that for functional errors, the actual fault location can be very far from the assert statement responsible for the unexpected output \cite{bohme2017bug}.

The example emphasizes an explicit point that {\em you can not locate the buggy method if you have not even seen it}. 
To remedy this, \toolname equips LLM with a lightweight program instrumentation mechanism for concentrating on the method call flow during test execution (upper right in Figure \ref{fig:motiv}).
Although it may still be non-trivial for LLMs to see the whole elephant, we argue that the method calls as a type of execution information could be helpful by highly summarizing the entire test behavior.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/motivation.pdf}
    \caption{Motivation example extracted from bug Lang-34.}
    \label{fig:motiv}
\end{figure}

{\bf Demand for Elaborate Debugging Logic.}
In addition to the undercover nature of the error location, another difficulty is rooted in the sophistication of the debugging logic.
Current research about debugging episodes and strategies of human developers  have found that the debugging process usually requires multiple steps and the union of different expertness \cite{alaboudi2021exploratory,layman2013debugging}.
As shown in the bottom right of Figure \ref{fig:motiv}, practitioners adopt various actions such as {\em offline analysis} (analyze an error trace or a core dump), {\em code comprehension} (build mental representation by read and understand the code), and {\em forward reasoning} (follow each computational step in the execution of the failing test) during a debugging process \cite{romero2007debugging,bohme2017bug}.
For each action, different professional knowledge from software architecture to software testing is indispensable.
However, the LLM-based fault localization approaches so far neither take into consideration the complicated debugging logic, nor value the role of distinct knowledge in specific actions.

Though fitting the genuine logic of practitioners is still a distant goal, \toolname tries to explore reasonable strategies for building the debugging logic of the LLMs.
Inspired by the concept of standard operating procedures (SOP) \cite{zhou2023agents}, \toolname decomposes a whole debugging task into multiple phases connected in series, where each phase is conducted by an agent with a certain type of expertise.

==> tables/discussion.tex <==
\begin{table}[!t]
\caption{The results of GRACE$_{DD}$ compared to \bftoolname.}
\centering
\label{tab:dis}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lr|R{14mm}R{14mm}R{14mm}}
\hline
\textbf{Project} & \textbf{\# Bugs} & \textbf{Top-1} & \textbf{Top-3} & \textbf{Top-5} \\ \hline
Chart & 26 & 13\phantom{0}\textcolor{darkred}{$\downarrow$3}\phantom{0}         & 17\phantom{0}\textcolor{darkred}{$\downarrow$1}\phantom{0}         & 17\phantom{0}\textcolor{darkred}{$\downarrow$2}\phantom{0}         \\
\rowcolor{grey} Lang & 65 & 33\phantom{0}\textcolor{darkred}{$\downarrow$11}        & 36\phantom{0}\textcolor{darkred}{$\downarrow$9}\phantom{0}         & 42\phantom{0}\textcolor{darkred}{$\downarrow$3}\phantom{0}         \\
Math & 106 & 35\phantom{0}\textcolor{darkred}{$\downarrow$14}        & 53\phantom{0}\textcolor{darkred}{$\downarrow$7}\phantom{0}         & 59\phantom{0}\textcolor{darkred}{$\downarrow$2}\phantom{0}         \\
\rowcolor{grey} Time & 27 & 9\phantom{0}\textcolor{darkred}{$\downarrow$2}\phantom{0}          & 14\phantom{0}\textcolor{darkgreen}{$\uparrow$1}\phantom{0}         & 14\phantom{0}\textcolor{darkgreen}{$\uparrow$1}\phantom{0}         \\
Mockito & 38 & 11\phantom{0}\textcolor{darkred}{$\downarrow$2}\phantom{0}         & 15\phantom{0}\textcolor{darkgreen}{$\uparrow$1}\phantom{0}         & 16\phantom{0}\textcolor{darkgreen}{$\uparrow$2}\phantom{0}         \\
\rowcolor{grey} Closure & 133 & 26\phantom{0}\textcolor{darkgreen}{$\uparrow$2}\phantom{0}         & 44\phantom{0}\textcolor{darkgreen}{$\uparrow$11}        & 48\phantom{0}\textcolor{darkgreen}{$\uparrow$13}        \\ \hline
Overall & 395 & 127\phantom{0}\textcolor{darkred}{$\downarrow$30}       & 179\phantom{0}\textcolor{darkred}{$\downarrow$4}\phantom{0}        & 196\phantom{0}\textcolor{darkgreen}{$\uparrow$9}\phantom{0}        \\ \hline
\end{tabular}
}
\end{table}
